Particle Physics and Cosmology

Today, both particle physics and cosmology are described by few parameter Standard Models, i.e. it is possible to deduce consequence of particle physics in cosmology and vice verse. The former is examined in this lecture, in light of the recent systematic exploration of the electroweak scale by the LHC experiments. The two main results of the first phase of the LHC, the discovery of a Higgs-like particle and the absence so far of new particles predicted by "natural" theories beyond the Standard Model (supersymmetry, extra-dimension and composite Higgs) are put in a historical context to enlighten their importance and then presented extensively. To be complete, a short review from the neutrino physics, which can not be probed at LHC, is also given. The ability of all these results to resolve the 3 fundamental questions of cosmology about the nature of dark energy and dark matter as well as the origin of matter-antimatter asymmetry is discussed in each case.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = LesHouchesPralavorioArXiv

default: testpdflatex

testpdflatex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	bibtex ${BASENAME} 
	pdflatex  ${BASENAME}
#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 



